Distributed Data Storage Systems with Opportunistic Repair

The reliability of erasure-coded distributed storage systems, as measured by the mean time to data loss (MTTDL), depends on the repair bandwidth of the code. Repair-efficient codes provide reliability values several orders of magnitude better than conventional erasure codes. Current state of the art codes fix the number of helper nodes (nodes participating in repair) a priori. In practice, however, it is desirable to allow the number of helper nodes to be adaptively determined by the network traffic conditions. In this work, we propose an opportunistic repair framework to address this issue. It is shown that there exists a threshold on the storage overhead, below which such an opportunistic approach does not lose any efficiency from the optimal storage-repair-bandwidth tradeoff; i.e. it is possible to construct a code simultaneously optimal for different numbers of helper nodes. We further examine the benefits of such opportunistic codes, and derive the MTTDL improvement for two repair models: one with limited total repair bandwidth and the other with limited individual-node repair bandwidth. In both settings, we show orders of magnitude improvement in MTTDL. Finally, the proposed framework is examined in a network setting where a significant improvement in MTTDL is observed.

==> discussions.tex <==
%\section{Special Cases}
%In this section, we will consider some special cases of the results described in the previous section.

\section{Generalized Degrees of Freedom Region of MIMO Interference Channel with Feedback}

This section describes our results on the GDoF region of the two-user MIMO IC with feedback. The GDoF gives the high SNR characterization of the capacity region. Since the inner and outer-bounds on the capacity region are within a constant gap, we characterize the exact GDoF region of the MIMO IC with feedback.

Define
\begin{eqnarray}\label{f}
f(u,\left({a}_{1},u_1\right),\left({a}_{2},u_2\right))\triangleq
\begin{cases}
\min{(u,u_1)}a^+_1+\min{((u-u_1)^+,u_2)}a_2^+, & \text{ if } a_1\ge a_2\\
\min{(u,u_2)}a^+_2+\min{((u-u_2)^+,u_1)}a_1^+, & \text{ otherwise }
\end{cases}.
\end{eqnarray}

The following result characterizes the GDoF for general MIMO IC with feedback for general power scaling parameters $\alpha_{ij}$.

\begin{theorem}
The GDoF region of the two-user MIMO IC with feedback is given by the set of $(d_1,d_2)$ satisfying:
\begin{eqnarray}
{\alpha }_{11}d_1&\le& f(N_1,\left({\alpha }_{11},M_1\right),\left({\alpha }_{21},M_2\right)),\label{gdofeq1}\\
{\alpha }_{22}d_2&\le& f(N_2,\left({\alpha }_{22},M_2\right),\left({\alpha }_{12},M_1\right)),\label{gdofeq2}\\
{\alpha }_{11}d_1&\le& {\alpha }_{12}{\min  \left(M_1,N_2\right)\ }+{\alpha }_{11}{\min  \left({\left(M_1-N_2\right)}^+,N_1\right)\ }+\nonumber\\
&&{\left({\alpha }_{11}-{\alpha }_{12}\right)}^+({\min  \left(M_1,N_1\right)\ }-{\min  \left({\left(M_1-N_2\right)}^+,N_1\right)\ }),\label{gdofeq3}\\
{\alpha }_{22}d_2&\le& {\alpha }_{21}{\min  \left(M_2,N_1\right)\ }+{\alpha }_{22}{\min  \left({\left(M_2-N_1\right)}^+,N_2\right)\ }+\nonumber\\
&&{\left({\alpha }_{22}-{\alpha }_{21}\right)}^+\left({\min  \left(M_2,N_2\right)\ }-{\min  \left({\left(M_2-N_1\right)}^+,N_2\right)\ }\right),\label{gdofeq4}\\
{\alpha }_{11}d_1+{\alpha }_{22}d_2&\le& f\left(N_2,\left({\alpha }_{22},M_2\right),\left({\alpha }_{12},M_1\right)\right)+{\alpha }_{11}{\min  \left({\left(M_1-N_2\right)}^+,N_1\right)\ }+\nonumber\\
&&{\left({\alpha }_{11}-{\alpha }_{12}\right)}^+\left({\min  \left(M_1,N_1\right)\ }-{\min  \left({\left(M_1-N_2\right)}^+,N_1\right)\ }\right),\label{gdofeq5}\\
{\alpha }_{11}d_1+{\alpha }_{22}d_2&\le& f\left(N_1,\left({\alpha }_{11},M_1\right),\left({\alpha }_{21},M_2\right)\right)+{\alpha }_{22}{\min  \left({\left(M_2-N_1\right)}^+,N_2\right)\ }+\nonumber\\
&&{\left({\alpha }_{22}-{\alpha }_{21}\right)}^+\left({\min  \left(M_2,N_2\right)\ }-{\min  \left({\left(M_2-N_1\right)}^+,N_2\right)\ }\right). \label{gdofeq6}
\end{eqnarray}

\label{thm_gdof}
\end{theorem}
\begin{proof}
According to Theorem \ref{outer_inner_capacity_reciprocal}, we can see that GDoF is equal to $\lim_{\mathsf{SNR}\to \infty}\mathcal{R}_o(0)/\log \mathsf{SNR} $. Appendix \ref{Appendix3} evaluates the limit of $\mathcal{R}_o(0)/\log \mathsf{SNR}$ as $\mathsf{SNR}\to \infty$ to get the result as in the statement of the Theorem.
\end{proof}
Since the capacity region of the MIMO IC with feedback and the corresponding reciprocal IC with feedback are within constant gap, the GDoF region of the MIMO IC with feedback and that of the corresponding reciprocal IC with feedback are the same, as given in the next corollary.
\begin{corollary}
The GDoF region for the reciprocal IC with feedback is given by the set of $(d_1,d_2)$ satisfying \eqref{gdofeq1}-\eqref{gdofeq6}.\label{cor:reciprocity}
\end{corollary}

We will now consider a special case of Theorem \ref{thm_gdof} where $M_1=M_2=M$, $N_1=N_2=N$, $\alpha_{11}=\alpha_{22}=1$, and $\alpha_{12}=\alpha_{21}=\alpha$. This MIMO IC is called a symmetric MIMO IC. We also define GDoF $d$ as the supremum over all $d_i$ such that $(d_i,d_i)$ is in the GDoF region. The GDoF for the symmetric MIMO IC with feedback is given as follows.

\begin{corollary}
The GDoF for a two-user symmetric MIMO IC with feedback for $N\le M$ is given as follows:
\begin{eqnarray}
GDoF_{PF}=\left\{ \begin{array}{ccc}
N-\frac{\alpha}{2} {\left(2N-M\right)}^+,& \text{ if }\alpha \le 1, \\
N(\frac{\alpha+1}{2})-\frac{1}{2}{\left(2N-M\right)}^+,& \text{ if } \alpha \ge 1. \end{array}
\right.
\end{eqnarray}
Since the expressions are symmetric in $N$ and $M$ by Corollary \ref{cor:reciprocity}, the GDoF for $M\le N$ follow by interchanging the roles of $M$ and $N$.
\end{corollary}
\begin{proof}
For the symmetric MIMO IC, we have
\begin{eqnarray}
f(N_i,\left({\alpha }_{ii},M_i\right),\left({\alpha }_{ji},M_j\right))&=&f(N,\left(1,M\right),\left({\alpha },M\right))\nonumber\\
&=& \max(1,\alpha)\min(M,N)+\min(1,\alpha)\min((N-M)^+,M).\label{fforsym}
\end{eqnarray}

Let the GDoF be $d$.  We will split the proof for $N\le M$ in two cases.

\noindent {\bf Case 1 - $\alpha\le1$:}
We will go over all equations \eqref{gdofeq1}-\eqref{gdofeq6} and evaluate them for the symmetric case with $\alpha\le 1$.
Equations (\ref{gdofeq1}) and (\ref{gdofeq2}) can be simplified using \eqref{fforsym} as follows
\begin{eqnarray}
d&\le& \max(1,\alpha)\min(M,N)+\min(1,\alpha)\min((N-M)^+,M)\nonumber\\
&=&N. \label{simp1l1}
\end{eqnarray}
Equations (\ref{gdofeq3}) and (\ref{gdofeq4}) can be simplified as
\begin{eqnarray}
d&\le& {\alpha }{\min  \left(M,N\right)\ }+{\min  \left({\left(M-N\right)}^+,N\right)\ }+{\left(1-{\alpha }\right)}^+({\min  \left(M,N\right)\ }-{\min  \left({\left(M-N\right)}^+,N\right)\ })\nonumber\\
&=& \alpha N+\min((M-N),N)+{(1-{\alpha })}{N}-{(1-\alpha)}{\min  \left({\left(M-N\right)},N\right)\ }\nonumber\\
&=&N+\alpha\min((M-N),N)\nonumber\\
&=&N+\alpha(N-(2N-M)^+). \label{simp2l1}
\end{eqnarray}
Equations (\ref{gdofeq5}) and (\ref{gdofeq6}) can be simplified as
\begin{eqnarray}
d&\le& \frac{1}{2}(\max(1,\alpha)\min(M,N)+\min(1,\alpha)\min((N-M)^+,M)+{\min  \left({\left(M-N\right)}^+,N\right)\ }+\nonumber\\
&&{\left(1-{\alpha }\right)}^+({\min  \left(M,N\right)\ }-{\min  \left({\left(M-N\right)}^+,N\right)\ }))\nonumber\\
&=&\frac{1}{2}(N+(1-\alpha)N+\alpha\min((M-N),N))\nonumber\\
&=&N-\frac{1}{2}\alpha(N-(N-(2N-M)^+))\nonumber\\
&=&N-\frac{\alpha}{2}((2N-M)^+).  \label{simp3l1}
\end{eqnarray}

We note that the minimum of the right hand sides of \eqref{simp1l1}, \eqref{simp2l1}, and \eqref{simp3l1} would give us the GDoF. The minimum of these three terms is \eqref{simp3l1} which proves the result for $\alpha \le 1$.


\noindent {\bf Case 2 - $\alpha\ge1$:}

In this case, equations (\ref{gdofeq1}) and (\ref{gdofeq2}) can be simplified as
\begin{eqnarray}
d&\le& \max(1,\alpha)\min(M,N)+\min(1,\alpha)\min((N-M)^+,M)\nonumber\\
&=&\alpha N. \label{simp1g1}
\end{eqnarray}
Equations (\ref{gdofeq3}) and (\ref{gdofeq4}) can be simplified as
\begin{eqnarray}
d&\le& {\alpha }{\min  \left(M,N\right)\ }+{\min  \left({\left(M-N\right)}^+,N\right)\ }+\nonumber\\
&&{\left(1-{\alpha }\right)}^+({\min  \left(M,N\right)\ }-{\min  \left({\left(M-N\right)}^+,N\right)\ })\nonumber\\
&=& \alpha N+\min((M-N),N). \label{simp2g1}
\end{eqnarray}
Equations (\ref{gdofeq5}) and (\ref{gdofeq6}) can be simplified as
\begin{eqnarray}
d&\le& \frac{1}{2}(\max(1,\alpha)\min(M,N)+\min(1,\alpha)\min((N-M)^+,M)+{\min  \left({\left(M-N\right)}^+,N\right)\ }+\nonumber\\
&&{\left(1-{\alpha }\right)}^+({\min  \left(M,N\right)\ }-{\min  \left({\left(M-N\right)}^+,N\right)\ }))\nonumber\\
&=&\frac{1}{2}(\alpha N+(N-(2N-M)^+))\nonumber\\
&=&N\frac{(\alpha+1)}{2}-\frac{1}{2}(2N-M)^+. \label{simp3g1}
\end{eqnarray}
We note that the minimum of the right hand sides of \eqref{simp1g1}, \eqref{simp2g1}, and \eqref{simp3g1} would give us the GDoF. The minimum of these three terms is \eqref{simp3g1} which proves the result for $\alpha \ge 1$.
\end{proof}

The authors of  \cite{gdof} found the GDoF for the two-user symmetric MIMO IC without feedback as follows for $N\le M$ (We can interchange the roles of $N$ and $M$ if $N>M$.)
\begin{eqnarray}
GDoF_{NF}=\left\{ \begin{array}{ccc}
N-{\alpha}{\left(2N-M\right)}^+,&  \text{ if }0\le\alpha\le\frac{1}{2},\\
N-(1-{\alpha}){\left(2N-M\right)}^+,& \text{ if }\frac{1}{2}\le\alpha\le \frac{2}{3} ,\\
N-\frac{\alpha}{2}{\left(2N-M\right)}^+,& \text{ if }\frac{2}{3}\le\alpha\le1,\\
\min\{N,N(\frac{\alpha+1}{2})-\frac{1}{2}{\left(2N-M\right)}^+\},& \text{ if } \alpha \ge 1 \end{array}
\right.
\end{eqnarray}

We note that the GDoF with and without feedback are the same for $\frac{2}{3}\le\alpha \le 1$. Figure \ref{fig:subfigureExample} compares the GDoF for the two-user symmetric MIMO IC with and without feedback. In Figure \ref{fig:subfigureExample}(a), the ``W"-curve obtained without feedback delineates the very weak ($0\le\alpha\le\frac{1}{2}$), weak ($\frac{1}{2}\le\alpha\le\frac{2}{3}$), moderate ($\frac{2}{3}\le\alpha\le1$), strong ($1\le\alpha\le{3-{\frac{M}{N}}}$) and very strong ($3-{\frac{M}{N}}\le\alpha$) interference regimes. In the presence of feedback, the ``W"-curve improves to a ``V"-curve which delineates the weak ($0\le\alpha\le1$) and strong ($1\le\alpha$) interference regimes for all choices of $N$ and $M$. For $\frac{M}{2}<N\leq M$, we see that the GDoF with feedback is strictly greater than that without feedback for $0<\alpha< 2/3$ and for $\alpha > 3-M/N$. For $N\le M/2$,  we see that the GDoF with feedback is strictly greater than that without feedback for $\alpha > 2$. The GDoF improvement indicates an unbounded gap in the corresponding capacity regions as the SNR goes to infinity.

%\begin{figure}[ht]
%\centering
%\subfigure[$\frac{M}{2}<N\leq M\quad\left(\alpha_0=3-\frac{M}{N}\Rightarrow 1<\alpha_0\leq2\right)$]{
%	\includegraphics[width=8.5cm]{1.pdf}
%    \label{fig:subfig1}
%}
%\subfigure[$N\leq \frac{M}{2}$]{
%	\includegraphics[width=8.5cm]{2.pdf}
%    \label{fig:subfig2}
%}
%\caption[Optional caption for list of figures]{GDoF for symmetric MIMO IC with perfect feedback (PF), and no-feedback (NF) for \subref{fig:subfig1} $\frac{M}{2}<N\leq M$, and \subref{fig:subfig2} $N\leq \frac{M}{2}$.}
%\label{fig:subfigureExample}
%\end{figure}
Interestingly, from Figure \ref{fig:subfigureExample}(b) we can see that if we increase $M$ when $N\leq\frac{M}{2}$, the GDoF does not change. This can be interpreted as that while $N\leq\frac{M}{2}$, $N$ act as a bottle-neck and increasing $M$ does not increase the GDoF. As a special case consider a MISO IC for which we note that the GDoF is the same for all $M\ge 2$. Thus, increasing the transmit antennas beyond $2$ does not increase the GDoF. However, increasing the transmit antennas from $1$ to $2$ gives a strict improvement in GDoF for all $\alpha>0$. Similar result also holds for SIMO systems where increasing the receive antennas from $1$ to $2$ help increase GDoF while increasing the receive antennas beyond $2$ does not increase the GDoF.




%\subsubsection{GDOF of the MISO Interference Channel with Feedback}

%In this part we express the channel and its inner and outer bound gap in MISO case. We can see GDoF plot for each $M=1,2,3$ in Figure 2. As we see, it increases by M.

%Surprisingly, we see that for every number of antennas in transmitters, the obtained gap between inner and outer bound is 2 bits.


==> exact_mbr.tex <==
\section{Exact Repair for a point based on MBR}

In this section, we will follow the product matrix based approach for exact repair in \cite{RashmiShah:11} to achieve the AMBR point. Normalizing the points with $\beta = (n_l-d_l)$, the parameters for MBR point are:

\begin{eqnarray}
\alpha &=& d'\\
\mathsf{M} &=& \left( {{k'+1} \choose 2}+k'(d'-k')\right),
\end{eqnarray}
where $k' = k (n_l-d_l)$ and $d'=(d_b+1)(n_l-d_l)-1$. 


Let $S$ be a $k' \times k'$ symmetric matrix constructed such that the upper triangular matrix is filled up by ${{k'+1} \choose 2}$ distinct message symbols drawn from the set $\{u_j\}_{j=1}^{{{k'+1} \choose 2}}$. The remaining $k'(d'-k')$ message symbols are filled in  matrix $T$ of size $k' \times (d'-k')$. The message matrix $M$ is then defined as the $d'\times d'$ symmetric matrix given by
\begin{equation}
M= \left[ \begin{array}{cc}
S & T \\
T^t & 0 \end{array} \right] .
\end{equation}
Next, we define the encoding matrix $\psi$ to be $n(n_l-d_l) \times d'$ matrix of the form
\begin{equation}
\psi= \left[ \begin{array}{cc}
\Phi & \Delta\end{array} \right] ,
\end{equation}
where $\Phi$ and $\Delta$ are $(n(n_l-k_l)\times k')$ and $(n(n_l-d_l)\times d'-k')$ matrices respectively satisfying some conditions as will be described later. Let the $n(n_l-d_l)$ rows of $\psi$ be denoted by $\psi_{1,1}, \cdots, \psi_{1,n_l-d_l}, \psi_{2,1}, \cdots \psi_{n,n_l-d_l}$ from top to bottom. Further, we denote
$\psi_i = \left[ \begin{array}{c}
\psi_{i,1} \\
\psi_{i,2} \\
\cdots \\
\psi_{i,n_l-d_l} \end{array} \right]$. Let
\begin{equation}
B= \left[ \begin{array}{c}
B_1 \\
B_2\\
\cdots \\
B_{n_l} \end{array} \right]
\end{equation}
be a $(n_l \times n_l-d_l)$ matrix where any  $n_l-d_l$ rows are linearly independent. We assume that the first $n_l-d_l$ rows of $B$ form an identity matrix. Then, $j^{\text{th}}$ disk in $i^{\text{th}}$ cluster is $B_j \left[ \begin{array}{c}
\psi_{i,1} \\
\psi_{i,2}\\
\cdots \\
\psi_{i,n_l-d_l} \end{array} \right] M$, for any $1\le i\le n$ and $1\le j\le n_l-d_l$. We assume the following conditions on $\psi$:
\begin{enumerate}
\item Any $k'$ rows of $\Phi$ are linearly independent.
\item For any $1\le i\le n$,  any $(j_1, \cdots j_{d_b})\in [1,n]\setminus \{i\} $, and any $(k_1, \cdots k_{n_l-d_l-1})\in [1,n_l]$, the rows  of
    $\left[ \begin{array}{c}
B_{k_1}\psi_{i,k_1} \\
\cdots \\
B_{k_{n_l-d_l-1}}\psi_{i,k_{n_l-d_l-1}} \\
\psi_{j_1} \\
\cdots \\
\psi_{j_{d_b}} \end{array} \right]$ are linearly independent.
\end{enumerate}

We note that all these conditions can be met due to Schwartz-Zippel lemma when the field-size is large enough. The next results show the exact regeneration and the data reconstruction properties of the code.

\begin{theorem}
In the code presented, exact-regeneration of any $d_l+1$ failed nodes in a cluster can be achieved by connecting to any $d$ of the remaining $n-1$ remaining clusters.
\end{theorem}
\begin{proof}
Let $d_l+1$ disks fail in cluster $i$. Then, out of the first $n_l-d_l$ systematic disks, at-least one of the disks would have failed. Without loss of generality, let that disk be the first one. Let $(k_1, \cdots k_{n_l-d_l-1})\in [2,n_l]$ be the disks that are not failed in cluster $i$. In this setting, we will now show that we can reconstruct this failed disk.

Each of the $d_b$ contacted disks $j_i$ contribute $\psi_{j_i} M \psi_{i,1}^t$, for $(j_1, \cdots j_{d_b})\in [1,n]\setminus \{i\}$. Thus, the first $n_l-d_l$ disks in a contacted cluster give 1 linear combination which satisfies $\beta = n_l-d_l$. Further, all the remaining disks in $i^{\text{th}}$ cluster are available. With this, the failed cluster has access to
$\left[ \begin{array}{c}
B_{k_1}\psi_{i,k_1} \\
\cdots \\
B_{k_{n_l-d_l-1}}\psi_{i,k_{n_l-d_l-1}} \\
\psi_{j_1} \\
\cdots \\
\psi_{j_{d_b}} \end{array} \right] M \psi_{i,1}^t$. Since the first matrix is $d'\times d'$ full-rank matrix and can be inverted, the failed disk has access to $\psi_{i,1} M$ (since $M$ is symmetric). Thus, the data of the failed disk is recovered. Now, in $i^{th}$ cluster, we have access to $n_l-d_l$ disks and thus the remaining can be reconstructed due to MDS property.
\end{proof}

\begin{theorem}
In the code presented, all the $M$ messages can be reconstructed by contacting $k$ clusters.
\end{theorem}
\begin{proof}
From the $k$ remaining clusters, say $i_1, \cdots i_k$, we form
$\psi_{left} = \left[ \begin{array}{c}
\psi_{i_1} \\
\cdots \\
\psi_{i_k} \end{array} \right]$. This matrix is made of $k'$ rows which is a block matrix with the corresponding $k'$ rows of $\Phi$ and $k'$ rows of $\Delta$. Let these sub-matrices of $\Phi$ and $\Delta$ be denoted by $\Phi_{left}$ and $\Delta_{left}$. Thus, $\psi_{left} M = \left[ \begin{array}{cc} \Phi_{left}S + \Delta_{left}T^t & \Phi_{left} T \end{array} \right]$. By construction, $ \Phi_{left}$ is non-singular. Thus, we can get $T$ from $\Phi_{left} T$ and then by subtracting $T$ term from  $\Phi_{left}S + \Delta_{left}T^t$, obtain $S$.
\end{proof}

We now consider one example of the above code construction. Let $n_b=5$, $k=2$, $d_b=3$, $n_l=3$, $d_l=1$. We choose $q=11$ so we are operating over $\mathbb{F}_{11}$. $B_3$ is taken to be $[1 1]$. Thus, each cluster has the third disk being the sum of the other two disks. Thus, a single disk failure in the cluster can be repaired locally. The matrix $\psi$ is taken to be Vandermonde matrix over $\mathbb{F}_{11}$ and is given as
\begin{equation}
\psi = \left[ \begin{array}{ccccccc}	1& 1& 1& 1& 1& 1& 1 \\
 1& 2& 4& 8& 5&10& 9 \\
 1& 3& 9& 5& 4& 1& 3 \\
 1& 4& 5& 9& 3& 1& 4 \\
 1& 5& 3& 4& 9& 1& 5 \\
 1& 6& 3& 7& 9&10& 5 \\
 1& 7& 5& 2& 3&10& 4 \\
 1& 8& 9& 6& 4&10& 3 \\
 1& 9& 4& 3& 5& 1& 9 \\
 1&10& 1&10& 1&10& 1
\end{array} \right]
\end{equation}
It can be verified that this $\psi$ satisfies all the desired conditions and thus forms a valid code.

==> exact_msr.tex <==
\section{Exact Repair for Minimum Storage Regenerating Point}

In this section, we will give the code designs for the minimum storage regenerating point. Although the product matrix framework of \cite{RashmiShah:11} can be extended to hierarchal storage, we do not explain that case here since this framework yields optimal codes only for $d\ge 2k-2$ in \cite{RashmiShah:11}. We however show below extension of the interference alignment based framework as in \cite{Cadambe:11}.

The approach for achieving MSR point follows the approach in \cite{Cadambe:11}. The $n_b(n_l-d_l)$ discs which correspond to $n_l-d_l$ disks in each cluster use similar coding as in \cite{Cadambe:11} where any $k(n_l-d_l)$ disks can be used to reconstruct the whole data. These disks are obtained, for example, from $k$ clusters. Each cluster has data for $n_l-d_l$ disks as defined by the above coding, and let cluster $i$ have data $x_{i,1} \cdots x_{i,n_l-d_l}$. The remaining disks $n_l-d_l<j\le n_l$ has data $\sum_{y=1}^{n_l-d_l}B_{i,j,y}x_{i,y}$ where all $B_{i,j,y}$ are diagonal matrices with random elements in the field on diagonal such that they form a MDS code due to which all the data in a cluster can be recovered from any $n_l-d_l$ disks in that cluster.  diagonal matrices with random elements on diagonal.  For regeneration, suppose that $n_l-d_l+1$ disks fail from cluster $i$. We assume that disks $1, n_l-d_l+1, \cdots, n_l-d_l$ fail. Thus, we repair disk $1$ using disks $2$ through $n_l-d_l$ of the same cluster and the first $n_l-d_l$ disks of the contacted $d_b$ clusters. The recovery conditions directly follow from the discussions in \cite{Cadambe:11}. After this repair $n_l-d_l$ disks are recovered in the failed cluster and thus the rest can be recovered. The conversion from systematic to non-systematic disks in the cluster can be done due to MDS property among the $n_l-d_l$ disks in the cluster and thus similar arguments in \cite{Cadambe:11} can be used to show the result for any $d_l+1$ failed disks in the cluster for a large enough field size. Thus, the following result follows.

\begin{theorem}
For message size $M$, and $\alpha = \frac{M}{k(n_l-d_l)}$, there is an exact repair code for which the access bandwidth from each cluster $\beta$ satisfies
\begin{equation}
\beta = \frac{M}{k(d_b+1-k)(n_l-d_l)}+o(M)
\end{equation}
\end{theorem}


%As an example, consider $n_b=4, d_b=3, k=2, n_l=4, d_l=1$. 
 

==> functional_results.tex <==
\section{Hierarchical Distributed Storage}\label{sec:functional}
In this section, we will describe our results for a hierarchical distributed storage system. The first result is the on the functional repair for the hierarchical distributed storage system.

\begin{theorem}
For any $\alpha \ge \alpha^*(n_b, n_l, k, d_b, d_l,\mathsf{M}, \gamma)$, the points $(n_b, n_l, k, d_b, d_l,\mathsf{M}, \alpha, \gamma)$ are feasible, and linear network codes suffice
to achieve them. It is information theoretically impossible to
achieve points with $\alpha < \alpha^*(n_b, n_l, k, d_b, d_l,\mathsf{M}, \gamma)$. The threshold function $\alpha^*(n_b, n_l, k, d_b, d_l,\mathsf{M}, \gamma)$ is the following:
\begin{equation}
\alpha^*(n_b, n_l, k, d_b, d_l,\mathsf{M}, \gamma) = \begin{cases}
\frac{M}{k(n_l-d_l)} & \gamma \in [\frac{1}{\frac{1}{f(0)}+ \frac{k(n_l-d_l-1)h(0)}{\mathsf{M}}},\infty)\\
\frac{M-g(i)\gamma}{k(n_l-d_l)-i} & \gamma \in [\frac{1}{\frac{1}{f(i)}+ \frac{k(n_l-d_l-1)h(i)}{\mathsf{M}}},\frac{1}{\frac{1}{f(i-1)}+ \frac{k(n_l-d_l-1)h(i-1)}{\mathsf{M}}}), 1\le i<k,\\
\frac{M-g(k)\gamma}{k(n_l-d_l-1)} & \gamma \in [0, \frac{1}{\frac{1}{f(k-1)}+ \frac{k(n_l-d_l-1)h(k-1)}{\mathsf{M}}}), \text {if } n_l-d_l>1
\end{cases}
\end{equation}
where
\begin{eqnarray}
f(i)&\triangleq& \frac{2\mathsf{M}d_b}{(2k-i-1)i+2k(d_b-k+1)}\\
g(i)&\triangleq& \frac{(2d_b-2k+i+1)i}{2d_b}\\
h(i)&\triangleq& \frac{d_b-k+1+i}{d_b}
\end{eqnarray}
\end{theorem}
\begin{proof}
This result is an extension of result in \cite{Dimakis:10}, with the main idea of the proof being that the code repair problem can be mapped to a multicasting problem on the information flow graph.

If $n_l-d_l=1$, the tradeoff is same as that in \cite{Dimakis:10}. This can be achieved by using the functional repair code in \cite{Dimakis:10} among the first disks of each cluster. Further, repetition code can be used among all the disks in the cluster. Thus, the rest of the proof focuses on the case when $n_l-d_l>1$.

Following similar analysis as in \cite{Dimakis:10}, we find that the min-cut from the source to the destination is given by \begin{equation}
\mathsf{C}\triangleq (n_l-d_l-1) k + \sum_{i=0}^{k-1} \min\{(d_b-i)\beta, \alpha\}.
\end{equation}

This is because each disk has content of $(n_l-d_l)\alpha$ since the rest of the cluster can be reconstructed from this. We replace each disk in \cite{Dimakis:10} with a cluster with storage of $(n_l-d_l)\alpha$. Further, on failure of $d_l+1$ disks in a cluster, for each cut before the input node, extra $(n_l-d_l-1)\alpha$ gets added to the cut doe to the remaining  $(n_l-d_l-1)$ disks which have not failed in the same cluster. Thus, similar analysis as in \cite{Dimakis:10} gives the above min-cut.

To ensure recoverability, we need $\mathsf{C}\ge \mathsf{M}$. We fix $\mathsf{M}$ and $\gamma$ to find
$\alpha^* (\mathsf{M},\gamma)$ which is defined as minimum value of $\alpha$ satisfying $\mathsf{C}\ge \mathsf{M}$. With the above min-cut and following similar analysis as in \cite{Dimakis:10} gives the result as in the statement of the Theorem. %We note that the last statement in the Theorem for lower $\gamma$ implies that the data can be recovered from the same cluster and thus incurs no access bandwidth.


Further, as noted in \cite{Dimakis:10}, there exists a
linear network code defined over a sufficiently large finite field (whose size depends on the graph size) such that all data collectors can recover the data object. Further, randomized
network coding guarantees that all collectors can recover the
data object with probability that can be driven arbitrarily high
by increasing the field size.
\end{proof}






We first note that for $n_l-d_l>1$, we have the minimum-bandwidth regenerating (MBR) point given by $(\alpha_{MBR},\gamma_{MBR}) = (\frac{M}{k(n_l-d_l-1)},0)$. This can be achieved by dividing the whole data into $k(n_l-d_l-1)$ disks constituting the first $n_l-d_l-1$ disks of $k$ clusters. An MDS code among these disks is used to fill the remaining first $n_l-d_l-1$ disks of remaining $n-k$ clusters. In each cluster, these $n_l-d_l-1$ disks are taken as systematic bits and an MDS code is used to fill the remaining $d_l+1$ disks. For the failure of $d_l+1$ disks, the MDS code in the cluster is used for repair. Further, from the first $n_l-d_l-1$ disks of any $k$ clusters, all the data can be recovered. Thus, this approach achieves the MBR point. Since MDS codes exist with probability 1 as the field size is large enough, this gives an exact repair to the MBR point.


%We first note that the first non-trivial point closest to MBR point corresponds to \[(\alpha_m, \gamma_m) = \left( \frac{M-g(k-1)\gamma_m}{k(n_l-d_l-1)+1}, \gamma_m\right),\]
%where $\gamma_m$ is given as
%\begin{eqnarray}
%\gamma_m&\triangleq&  \frac{1}{\frac{1}{f(k-1)}+ \frac{k(n_l-d_l-1)h(k-1)}{\mathsf{M}}}\\
%&=&  \frac{1}{\frac{k(k-1)+2k(d_b-k+1)}{2\mathsf{M}d_b}+ \frac{k(n_l-d_l-1)}{\mathsf{M}}}\\
%&=&  \frac{2\mathsf{M}d_b}{k(k-1)+2k(d_b-k+1)+ 2d_bk(n_l-d_l-1)}\\
%&=&  \frac{2\mathsf{M}d_b}{2kd_b(n_l-d_l) + k(k-1)-2k(k-1) }\\
%&=&  \frac{2\mathsf{M}d_b}{2kd_b(n_l-d_l) - k(k-1) }.
%\end{eqnarray}
%
%Further, it is easy to verify that $\frac{M-g(k-1)\gamma_m}{k(n_l-d_l-1)+1} = \frac{2\mathsf{M}d_b}{2kd_b(n_l-d_l) - k(k-1) }$. Thus, this point is given by
%\[(\alpha_m,\gamma_m)=\left(\frac{2\mathsf{M}d_b}{2kd_b(n_l-d_l) - k(k-1) }, \frac{2\mathsf{M}d_b}{2kd_b(n_l-d_l) - k(k-1) }\right).\] We note that $\alpha$ at this point is smaller than $\frac{M}{k(n_l-d_l-1)}$ for $n_l-d_l>1$ and thus the above gives a complete tradeoff.




We will now describe the extremal point corresponding to the best storage efficiency. We call the codes that achieve this point as the minimum-storage regenerating (MSR) codes.


For the MSR point, we see that $(\alpha_{MSR}, \gamma_{MSR}) = (\frac{M}{k(n_l-d_l)}, \frac{1}{\frac{1}{f(0)}+ \frac{k(n_l-d_l-1)h(0)}{\mathsf{M}}})$. This can be further simplified to see that the minimum storage point is achieved by the pair
\[(\alpha_{MSR}, \gamma_{MSR}) = \left( \frac{\mathsf{M}}{k(n_l-d_l)}, \frac{\mathsf{M}d_b}{k(d_b-k+1)(n_l-d_l)}\right).\]

The MSR point can be asymptotically achieved for exact regeneration. More precisely, we have
\begin{lemma}\label{msr} The minimum repair bandwidth $B_d$ for exact regeneration in a $(n, k, n_l, d_l, d_b)$ distributed
storage system satisﬁes
\[\alpha = \frac{\mathsf{M}}{k(n_l-d_l)}\]
\[\lim_{M \to \infty} \frac{B_d}{M} = \frac{d_b}{k(d_b-k+1)(n_l-d_l)} \]
\end{lemma}
\begin{proof}
For achievablity, we divide the whole content $M$ into $n_l-d_l$ sub-blocks, each of size $M/(n_l-d_l)$. For the first disks in each cluster, use the first sub-block and divide them in $n$ disks using the structure of \cite{Cadambe:11} such that the data can be recovered from any $k$ disks and repaired from $d_b$ disks. We repeat this for all the $n_l-d_l$ sub-blocks. For the remaining disks in the cluster, we use $(n_l, n_l-d_l)$ systematic MDS code to find the data in the remaining $d_l$ disks in the cluster.

We note that the recovery holds from any $k$ clusters since the systematic information in each sub-block can be recovered and then MDS code in the cluster can be used to recover the rest of the data. For repair of $d_l+1$ disks, we repair one of the failed systematic disks using the strategy in \cite{Cadambe:11} thus giving the repair bandwidth as in the statement of the Lemma. After this one repair, we use the MDS code inside the cluster to repair the remaining $d_l$ disks.
\end{proof}

In this paper, we will also explore another achievable point in the tradeoff which is denoted by $(\alpha_{AMBR},\gamma_{AMBR})$ and is given as
%The minimum repair bandwidth point is achieved by the pair
%Let $k' = k (n_l-d_l)$ and $d'=(d_b+1)(n_l-d_l)-1$. We first note that $d'-k'+1 = (n_l-d_l)(d_b-k+1)$. Thus,
\[(\alpha_{AMBR}, \gamma_{AMBR}) = \left( \frac{2\mathsf{M}d'}{(2k'd'-k'^2+k')}, \frac{2\mathsf{M}d_b(n_l-d_l)}{2k'd'-k'^2+k'}\right),\]
where $k' = k (n_l-d_l)$ and $d'=(d_b+1)(n_l-d_l)-1$. The parameters of this achievable point in the hierarchical distributed storage model have been chosen as an extension to the minimum-bandwidth regenerating (MBR) point in \cite{Dimakis:10}.

In the rest of this section, we will follow the product matrix based approach for exact repair in \cite{RashmiShah:11} to achieve the AMBR point. Normalizing the points with $\beta = (n_l-d_l)$, the parameters for MBR point are:

\begin{eqnarray}
\alpha &=& d'\\
\mathsf{M} &=& \left( {{k'+1} \choose 2}+k'(d'-k')\right),
\end{eqnarray}
where $k' = k (n_l-d_l)$ and $d'=(d_b+1)(n_l-d_l)-1$.


Let $S$ be a $k' \times k'$ symmetric matrix constructed such that the upper triangular matrix is filled up by ${{k'+1} \choose 2}$ distinct message symbols drawn from the set $\{u_j\}_{j=1}^{{{k'+1} \choose 2}}$. The remaining $k'(d'-k')$ message symbols are filled in  matrix $T$ of size $k' \times (d'-k')$. The message matrix $M$ is then defined as the $d'\times d'$ symmetric matrix given by
\begin{equation}
M= \left[ \begin{array}{cc}
S & T \\
T^t & 0 \end{array} \right] .
\end{equation}
Next, we define the encoding matrix $\psi$ to be $n(n_l-d_l) \times d'$ matrix of the form
\begin{equation}
\psi= \left[ \begin{array}{cc}
\Phi & \Delta\end{array} \right] ,
\end{equation}
where $\Phi$ and $\Delta$ are $(n(n_l-k_l)\times k')$ and $(n(n_l-d_l)\times d'-k')$ matrices respectively satisfying some conditions as will be described later. Let the $n(n_l-d_l)$ rows of $\psi$ be denoted by $\psi_{1,1}, \cdots, \psi_{1,n_l-d_l}, \psi_{2,1}, \cdots \psi_{n,n_l-d_l}$ from top to bottom. Further, we denote
$\psi_i = \left[ \begin{array}{c}
\psi_{i,1} \\
\psi_{i,2} \\
\cdots \\
\psi_{i,n_l-d_l} \end{array} \right]$. Let
\begin{equation}
B= \left[ \begin{array}{c}
B_1 \\
B_2\\
\cdots \\
B_{n_l} \end{array} \right]
\end{equation}
be a $(n_l \times n_l-d_l)$ matrix where any  $n_l-d_l$ rows are linearly independent. We assume that the first $n_l-d_l$ rows of $B$ form an identity matrix. Then, $j^{\text{th}}$ disk in $i^{\text{th}}$ cluster is $B_j \left[ \begin{array}{c}
\psi_{i,1} \\
\psi_{i,2}\\
\cdots \\
\psi_{i,n_l-d_l} \end{array} \right] M$, for any $1\le i\le n$ and $1\le j\le n_l-d_l$. We assume the following conditions on $\psi$:
\begin{enumerate}
\item Any $k'$ rows of $\Phi$ are linearly independent.
\item For any $1\le i\le n$,  any $(j_1, \cdots j_{d_b})\in [1,n]\setminus \{i\} $, and any $(k_1, \cdots k_{n_l-d_l-1})\in [1,n_l]$, the rows  of
    $\left[ \begin{array}{c}
B_{k_1}\psi_{i,k_1} \\
\cdots \\
B_{k_{n_l-d_l-1}}\psi_{i,k_{n_l-d_l-1}} \\
\psi_{j_1} \\
\cdots \\
\psi_{j_{d_b}} \end{array} \right]$ are linearly independent.
\end{enumerate}

We note that all these conditions can be met due to Schwartz-Zippel lemma when the field-size is large enough. The next results show the exact regeneration and the data reconstruction properties of the code.

\begin{theorem}
In the code presented, exact-regeneration of any $d_l+1$ failed nodes in a cluster can be achieved by connecting to any $d$ of the remaining $n-1$ remaining clusters.
\end{theorem}
\begin{proof}
Let $d_l+1$ disks fail in cluster $i$. Then, out of the first $n_l-d_l$ systematic disks, at-least one of the disks would have failed. Without loss of generality, let that disk be the first one. Let $(k_1, \cdots k_{n_l-d_l-1})\in [2,n_l]$ be the disks that are not failed in cluster $i$. In this setting, we will now show that we can reconstruct this failed disk.

Each of the $d_b$ contacted disks $j_i$ contribute $\psi_{j_i} M \psi_{i,1}^t$, for $(j_1, \cdots j_{d_b})\in [1,n]\setminus \{i\}$. Thus, the first $n_l-d_l$ disks in a contacted cluster give 1 linear combination which satisfies $\beta = n_l-d_l$. Further, all the remaining disks in $i^{\text{th}}$ cluster are available. With this, the failed cluster has access to
$\left[ \begin{array}{c}
B_{k_1}\psi_{i,k_1} \\
\cdots \\
B_{k_{n_l-d_l-1}}\psi_{i,k_{n_l-d_l-1}} \\
\psi_{j_1} \\
\cdots \\
\psi_{j_{d_b}} \end{array} \right] M \psi_{i,1}^t$. Since the first matrix is $d'\times d'$ full-rank matrix and can be inverted, the failed disk has access to $\psi_{i,1} M$ (since $M$ is symmetric). Thus, the data of the failed disk is recovered. Now, in $i^{th}$ cluster, we have access to $n_l-d_l$ disks and thus the remaining can be reconstructed due to MDS property.
\end{proof}

\begin{theorem}
In the code presented, all the $M$ messages can be reconstructed by contacting $k$ clusters.
\end{theorem}
\begin{proof}
From the $k$ remaining clusters, say $i_1, \cdots i_k$, we form
$\psi_{left} = \left[ \begin{array}{c}
\psi_{i_1} \\
\cdots \\
\psi_{i_k} \end{array} \right]$. This matrix is made of $k'$ rows which is a block matrix with the corresponding $k'$ rows of $\Phi$ and $k'$ rows of $\Delta$. Let these sub-matrices of $\Phi$ and $\Delta$ be denoted by $\Phi_{left}$ and $\Delta_{left}$. Thus, $\psi_{left} M = \left[ \begin{array}{cc} \Phi_{left}S + \Delta_{left}T^t & \Phi_{left} T \end{array} \right]$. By construction, $ \Phi_{left}$ is non-singular. Thus, we can get $T$ from $\Phi_{left} T$ and then by subtracting $T$ term from  $\Phi_{left}S + \Delta_{left}T^t$, obtain $S$.
\end{proof}

We now consider one example of the above code construction. Let $n_b=5$, $k=2$, $d_b=3$, $n_l=3$, $d_l=1$. We choose $q=11$ so we are operating over $\mathbb{F}_{11}$. $B_3$ is taken to be $[1 1]$. Thus, each cluster has the third disk being the sum of the other two disks. Thus, a single disk failure in the cluster can be repaired locally. The matrix $\psi$ is taken to be Vandermonde matrix over $\mathbb{F}_{11}$ and is given as
\begin{equation}
\psi = \left[ \begin{array}{ccccccc}	1& 1& 1& 1& 1& 1& 1 \\
 1& 2& 4& 8& 5&10& 9 \\
 1& 3& 9& 5& 4& 1& 3 \\
 1& 4& 5& 9& 3& 1& 4 \\
 1& 5& 3& 4& 9& 1& 5 \\
 1& 6& 3& 7& 9&10& 5 \\
 1& 7& 5& 2& 3&10& 4 \\
 1& 8& 9& 6& 4&10& 3 \\
 1& 9& 4& 3& 5& 1& 9 \\
 1&10& 1&10& 1&10& 1
\end{array} \right]
\end{equation}
It can be verified that this $\psi$ satisfies all the desired conditions and thus forms a valid code.



We will now extend the construction in \cite{Chao} to give a new code construction. The code in \cite{Chao} can be used in the first $n_l-d_l$ disks of each cluster followed by parity inside cluster as in Lemma \ref{msr}. The complete block designs achieve the code parameters as given below. 

\begin{eqnarray}
\alpha &=& \frac{d_b}{r-n_b+d_b}\beta\\
\mathsf{M} &=& \left(\frac{n_bd_b}{r} - \frac{d_bT_c}{(r+d_b-n_b)\binom{n_b-1}{r-1}}\right)(n_l-d_l)\beta,
\end{eqnarray}
for any $r$ satisfying $n_b-d_b+1\le r \le n_b-d_b + \frac{d_b}{d_b-k+1}$, and where $T_c = \sum_{i=n_b-d_b+1}^{\min(r,n_b-k)}(i+n_b-d_b) \binom{n-k}{i}\binom{k}{r-i} $. It is easy to see that this code construction achieves the asymptotic optimality in $n_b$ as proposed in \cite{Chao} for constant $n_l$, $d_l$, and for $k=n_b-\tau_1$ and $d_b = n-\tau_2$ where $\tau_1$ and $\tau_2$ are fixed positive integers with $\tau_1>\tau_2$.

